Assessment of a high-order shock-capturing central-difference scheme for hypersonic turbulent flow simulations

High-speed turbulent flows are encountered in most space-related applications (including exploration, tourism and defense fields) and represent a subject of growing interest in the last decades. A major challenge in performing high-fidelity simulations of such flows resides in the stringent requirements for the numerical schemes to be used. These must be robust enough to handle strong, unsteady discontinuities, while ensuring low amounts of intrinsic dissipation in smooth flow regions. Furthermore, the wide range of temporal and spatial active scales leads to concurrent needs for numerical stabilization and accurate representation of the smallest resolved flow scales in cases of under-resolved configurations. In this paper, we present a finite-difference high-order shock-capturing technique based on Jameson's artificial diffusivity methodology. The resulting scheme is ninth-order-accurate far from discontinuities and relies on the addition of artificial dissipation close to large gradients. The shock detector is slightly revised to enhance its selectivity and avoid spurious activations of the shock-capturing term. A suite of test cases ranging from 1D to 3D configurations (namely, shock tubes, Shu-Osher problem, isentropic vortex advection, under-expanded jet, compressible Taylor-Green Vortex, supersonic and hypersonic turbulent boundary layers) is analysed in order to test the capability of the proposed numerical strategy to handle a large variety of problems, ranging from calorically-perfect air to multi-species reactive flows. Results obtained on under-resolved grids are also considered to test the applicability of the proposed strategy in the context of implicit Large-Eddy Simulations.

==> blasius.tex <==
\section{Locally self-similar solution for laminar boundary layers}
\label{app:blasius}
\noindent The boundary-layer equations for a steady, compressible, multicomponent, reacting, two-dimensional flow (without pressure gradient) write:

% \noindent \textit{Global continuity:}
\begin{equation}
 \frac{\partial (\rho u)}{\partial x} + \frac{\partial (\rho v)}{\partial y} = 0
\end{equation}
% \noindent \textit{Species continiuty:}
\begin{equation}
 \rho u \frac{\partial Y_n}{\partial x} + \rho v \frac{\partial Y_n}{\partial y} = \frac{\partial}{ \partial y}\left(\rho_n u^D_n\right) + \dot{\omega}_n
\end{equation}
% \noindent \textit{x-Momentum:}
\begin{equation}
 \rho u \frac{\partial u}{\partial x} + \rho v \frac{\partial u}{\partial y} = \frac{\partial}{\partial y}\left(\mu \frac{\partial u }{\partial y} \right)
\end{equation}
% \noindent \textit{y-Momentum:}
% \begin{equation}
%  \frac{\partial p }{\partial y} = 0
% \end{equation}
% \noindent \textit{Total enthalpy conservation:}
\begin{equation}
 \rho u \frac{\partial h_0}{\partial x} + \rho v \frac{\partial h_0}{\partial y} = \frac{\partial}{\partial y }\left(\kappa \frac{\partial T}{\partial y} \right) + \frac{\partial}{\partial y}\left( \sum_n \rho_n u^D_n h_n \right) +  \left(\mu u \frac{\partial u}{\partial y}\right)
\end{equation}

\noindent where $h_0=h + u^2/2$ is the stagnation enthalpy. Independent variable transformations are introduced as follows (see Ref. \cite{lees1956laminar}):

\begin{equation}
\xi = \rho_e \mu_e U_e x = \xi(x), \qquad \eta = \frac{u_e}{\sqrt{2 \xi}} \int_0^y \rho dy= \eta (x,y).
\end{equation}
\noindent Considering the definition of the stream-function:
\begin{equation}
\frac{ \partial \psi}{ \partial y} = \rho u \qquad  \frac{ \partial \psi}{ \partial x} = - \rho v
\end{equation}
\noindent and the equivalent expression in terms of transformed variables

\begin{equation}
\frac{\partial \psi}{\partial \xi} = \frac{1}{\sqrt{2 \xi}}f(\eta) \quad \frac{\partial \psi}{\partial \eta} = \sqrt{2 \xi} f'(\eta),
\end{equation}

\noindent with $f'=u/u_e$, one can manipulate the boundary-layer equations and obtain their formulation in the self-similar coordinate system:

\begin{equation}
\left(Cf''\right)'+ff'' = 0
\end{equation}
\begin{equation}
\left[\frac{\rho^2 D_n}{\rho_e \mu_e}Y_n\left(\frac{X'_n}{X_n} -\sum_{i=1}^{NS}\frac{D_i}{D_n} \frac{Y_i}{X_i}X_i'\right)\right]' + fY'_n+ \frac{2 \xi \dot{\omega}_n/\rho}{\rho_e \mu_e u_e^2 } = 0
\label{eq:species}
\end{equation}

\begin{equation}
\frac{T_e}{h_{0,e}}\left(\frac{C \lambda}{\mu}\theta'\right)' +fg' + \frac{u_e^2}{h_{0,e}}\left( Cf'f''\right)'+\left[\sum_{n=1}^{NS} \frac{h_n}{h_{0,e}} \frac{\rho^2 D_n}{\rho_e \mu_e}Y_n\left(\frac{X'_n}{X_n} -\sum_{i=1}^{NS}\frac{D_i}{D_n} \frac{Y_i}{X_i}X_i'\right)\right]'= 0
\end{equation}

 \noindent Here, $g=h/h_{0,e}$ is the self-similar parameter for the enthalpy, whereas $\theta = T/T_e$; in addition, $C=\rho \mu/\rho_e \mu_e$ is the Chapman-Rubesin parameter. For the sake of clarity, in case of frozen chemistry or chemical equilibrium, the only $\xi$-dependent term in equation~\ref{eq:species} vanishes and the resulting equations become globally self-similar.
 The previous system of equations can be integrated numerically, subjected to the following boundary conditions:

 $$
 f'=f=0 \quad Y'_n=0 \quad g'=0, \quad \text{for} \quad \eta=0
 $$
 $$
 f'=1 \quad Y_n=Y_{n,e} \quad g=1-\frac{1}{2}\frac{u_e^2}{h_{0,e}}, \quad \text{for} \quad \eta \rightarrow \infty.
 $$

\noindent Considering a distance from the leading edge equal to $x=\SI{0.01}{m}$, we obtain the inflow profiles of normalized temperature, normalized velocity and species mass fractions, shown in figure~\ref{fig:blasius1} as a function of the incompressible similitude variable $\eta_i=y \sqrt{Re_x}/x$. Moreover, figure~\ref{fig:blasius2} displays the evolution of $C_f$ as a solution of the Navier-Stokes equations, compared with the results obtained from the aforementioned equations.

\begin{figure}[!h]
   \centering
     \begin{tikzpicture}
      \node[anchor=south west,inner sep=0] (a) at (0,0) {\includegraphics[width=0.44\columnwidth, trim={5 5 5 5}, clip]{thermo.eps}};
      \begin{scope}[x={(a.south east)},y={(a.north west)}]
        \node [align=center] at (0.56,0.0) {$\eta_i$};
        \node [align=center,rotate=90] at (-0.01,0.54) {$u/u_e$};
        \node [align=center,rotate=270] at (1.01,0.53) {$T/T_e$};
        \node [align=center] at (0.25,0.44) {$\longleftarrow$};
        \node [align=center] at (0.50,0.48) {$\longrightarrow$};
      \end{scope}
  \end{tikzpicture}
     \begin{tikzpicture}
      \node[anchor=south west,inner sep=0] (a) at (0,0) {\includegraphics[width=0.44\columnwidth, trim={5 5 5 5}, clip]{species.eps}};
      \begin{scope}[x={(a.south east)},y={(a.north west)}]
        \node [align=center] at (0.56,0.0) {$\eta_i$};
      \end{scope}
  \end{tikzpicture}
\caption{Evolution of normalized velocity and normalized temperature (left) and species mass fractions (right), at the inflow. $Y_{N_2}$ and $Y_{O_2}$ are not shown being outside the range.}
\label{fig:blasius1}
\end{figure}

\begin{figure}[!h]
   \centering
   \begin{tikzpicture}
      \node[anchor=south west,inner sep=0] (a) at (0,0) {\includegraphics[width=0.44\columnwidth, trim={5 5 5 5}, clip]{cf.eps}};
      \begin{scope}[x={(a.south east)},y={(a.north west)}]
        \node [align=center] at (0.58,0.0) {$(x-x_0)/\delta^*_\text{in}$};
        \node [align=center,rotate=90] at (-0.02,0.56) {$C_f$};
      \end{scope}
  \end{tikzpicture}
\caption{Evolution of skin friction coefficient obtained from Navier-Stokes equations (line) and from locally self-similar solution (symbols).}
\label{fig:blasius2}
\end{figure}

